Reinforcement Learning based Interconnection Routing for Adaptive Traffic Optimization

Applying Machine Learning (ML) techniques to design and optimize computer architectures is a promising research direction. Optimizing the runtime performance of a Network-on-Chip (NoC) necessitates a continuous learning framework. In this work, we demonstrate the promise of applying reinforcement learning (RL) to optimize NoC runtime performance. We present three RL-based methods for learning optimal routing algorithms. The experimental results show the algorithms can successfully learn a near-optimal solution across different environment states. Reproducible Code: github.com/huckiyang/interconnect-routing-gym

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> sections/02-RelatedWork.tex <==
\textbf{Efforts to Optimize NoC Routing}
Once the topology of a NoC is decided, we need routing algorithms to get high-performance and provide deadlock-freedom. Routing algorithms for NoCs have been studied for decades~\cite{glass1992turn, chiu2000odd, rantala2006network,jiang2009indirect, aydogan1996adaptive,chemli2014turn}.
%Turn models become a popular way to achieve a deadlock-free network in a mesh topology. It restricts the routers from certain turns to keep the network from looped dependency. For example, in a xy-turn model, each router can only take the x-direction first to reach the destination. Likewise, in a west-first model, the router needs to route the packet to the west port first. Dally et al. \cite{dally1986torus} develops the routing algorithms for torus topology. For more complex topology, some advanced routing algorithm is addressed %\cite{jiang2009indirect, guan1993analytical, aydogan1996adaptive}
%\cite{jiang2009indirect, aydogan1996adaptive}. 
%In the novel 3D technology, Chemli et, al. \cite{chemli2014turn} utilize novel turn model to avoid deadlock conflicts. 
%
Routing algorithms can be classified into three categories. First, deterministic routing (e.g., XY)
%\cite{adve1994performance,flich2012survey}
always choose the same route no matter what network condition it faces. This simple technique is widely applied in real NoC design because of its easy to implement characteristic. Second, Oblivious routing 
%\cite{towles2002worst,domke2011deadlock}
, which follows certain defined turn-model regardless of the network state. For example, a routing algorithm that randomly chooses between available deadlock-free routes is in this category. Third, adaptive routing, which not only follows a certain turn-model, but also considers the current network stats. 
\\
\vspace{+4pt}
\noindent\textbf{Contributions of this work:}
\vspace{-4pt}
\begin{itemize}
    \item We propose a reinforcement learning-based protocol to maximize the objective throughput of ICNs. 
    %In this method, we exploit the RL based models including Q-learning, SARSA, Expected-SARSA models to automate part of the traditional treatment procedure. 

    
    % \item We propose a localized buffer-level intelligent arrangement via EA with Genetic Algorithm, CMA-ES, and Parameter-Exploring Policy Gradients.  
    \item Besides, we incorporate the system-level utility function to evaluate the performance with the cost of power and training time. 
\end{itemize}

\noindent
% \subsubsection{NoC Routing via Machine Learning}
% In the area of ICNs, deep learning (DL) has gained more and more attention in recent years. Researchers have started applying novel DL algorithms to conventional NOC problems. Examples include handling 
% communication among modules which are dynamically placed on reconfigurable NoCs~\cite{boyan1994packet},
% Q-learning to find 
% optimal routing algorithms for bufferless NoCs~\cite{daya2016quest}, RL applied to learn an evolving deflection algorithm~\cite{feng2010reconfigurable}, and machine learning to provide guaranteed service at a low costs~\cite{daya2017low}.
%  We beleive RL can further improve routing performance by utilizing both local and global latencies with policy exploration, as we show in this work.

%Reinforcement-learning based approaches have not been comprehensively investigated in NoCs.


%the routing algorithm for bufferless NoC can be adjusted at run time. The Q-Learning is utilized to find optimal routing algorithm in different situation \cite{daya2016quest}. The deflection routing algorithm which reacts to the different level of congestion rate by configuring the new injection rate in each node. RL applied to learn an evolving deflection algorithm \cite{feng2010reconfigurable}. Also, Daya et al. \cite{daya2017low} use machine learning in the bufferless network architecture to provide guaranteed service at a low cost.

% \\
% \textbf{Efforts to Optimize Virtual Channel Placement and Allocation}
% Most virtual channel routers have multiple virtual channels to mitigate deadlock and achieve better performance. The static virtual channel allocation method could be applied to achieve better throughput by monitoring the congestion rate of each link \cite{huang2007virtual}. Also, Shim et, al. \cite{shim2009static} utilize a static method to allocate virtual channels with no deadlock oblivious of routing algorithm. Another branch is to use dynamic virtual channels allocation. The number of virtual channel in each link is decided according to the network rate \cite{lai2008dynamically}. Meanwhile, the scheme in \cite{xu2010simple} assigns virtual channels based on the designated output port of a packet to reduce the Head-of-Line (HoL) blocking. Many related works %\cite{nicopoulos2006vichar, dobkin2007qnoc, dally1993deadlock}
% \cite{nicopoulos2006vichar, dobkin2007qnoc}
% also utilize different aspects of network states to address the virtual channel allocation problem. 

% Most of the adaptive methods for allocating virtual channels utilize pre-collected statics of network traffic. However, in the real NoC environment, the network can change variable with time. The network traffic is unknown, and the network stats is not pre-obtainable. Then the pre-trained system cannot maintain high performance in the long term in this real-life dynamically changing environment scenario. We could possibly retrain the whole virtual channel configuration by new statistic data. However, the overhead for retraining is significant. Furthermore, the model is then only optimized for some earlier network traffic, which not necessarily reflect the current network state.
%We are not aware of NoC research that leverages ML techniques for efficient VC/buffer management.



==> sections/06-Discussion.tex <==
% \section{Discussion}
% \subsection{Training Time}
% The overhead of a learning agent is the runtime of this learning method. The system we use is an Intel Xeon Platium 8164 CPU, 2.00 GHz with 26 cores. Our baseline system is a 64 nodes mesh Garnet 2.0\cite{agarwal2009garnet}. The runtime for one episode is recorded in Table \ref{table:time}. The runtime of episodes depends on the number of iterations (or state transitions). One iteration of gem5\cite{binkert2011gem5} without any training algorithm takes about 12 msec. For S1, we have 9 state transition in one episode, so each run of S1 takes 18 msec for SARSA and 19.8 msec for QL. That is to say, the reinforcement training part takes around 33\% of the runtime for SARSA and 40 \% of runtime for QL. QL is more massive than SARSA. E-SARSA runtime percentage can be inducted in the same way.


% For Module 2 dynamic traffic, we have seven transitions, so the time for QL, SARSA, and E-SARSA is 19.65, 19.08, 19.98 respectively. E-SARSA has the most complexity. For module 2 in VC allocation, we have 11 population in one episode. Therefore, the one runtime for GA is 13.38 and for 14.42 for CMAES. Therefore ES one population training time ratio is 10.3 \% for GA and 16.8\% for CMAES. It is obvious that CMAES has higher complexity. For module 3, we use the same setting, and the trends are similar.

% Overall, for the performance, We find QL has the best performance; however, from the above analysis it also has the most runtime. As for ES, CMAES performs better than GA. However, CMAES takes more time as well. It shows for different application and needs, we could trade-off between performance and training time. 

% However, we should notice that the higher the performance gain also indicate the better efficiency of the learning algorithm. Therefore, even though it could take longer for one iteration, however, it could take less repetition to converge to the right solution.


% \input {table/time.tex}




% \subsection{Hardware Cost}
% We consider the hardware cost of the system that is implemented with the learning policy-based router. For the scenario with dynamic traffic, the extra cost is an SRAM, whose number of entry is the number of states in the environment. Therefore, if we use 32-bit width SRAM. Then for S1, it is $9\times32$ bits SRAM, for S2, it is $7\times32$ bits SRAM. They are very small SRAM compared to the whole router architecture.

% For the scenario with dynamic VC allocation. The extra cost is an SRAM, whose number of entry is the number of the port router has. Each entry recorders the stater address of the buffer of one port. Therefore, for S2 and S3, we have four ports that are implemented with dynamic VC. Then, we need a $4\times32$bits SRAM. For this scenario, we can quickly notice the benefit of this policy-based router by examining some traffic cases. Assumed we have a router with 16 dynamic allocable VC, and one of the routers is in a traffic pattern that will only have West-East direction packets. Then our learned policy-based router, it will allocate the VC as [0, 8, 0, 8], while the normal (baseline) router will obliviously allocate the VC as [4, 4, 4, 4]. However, the VC in North and South port are wasted for the baseline router. We can define the effective baseline router as the router with a larger total VC that can achieve the same performance as the learned policy-based router. For the above West-East Traffic example, the effective baseline router will need 32 VC totally, that is [8, 8, 8, 8] for each port. To simplify the comparison, let's assume we have a straightforward system with each VC just with one packet buffer. We compute their additional cost ratio ($CostRatio_{addition}$) as
% \begin{equation}
% CostRatio_{addition} = \frac{Cost_{system} - Cost_{baseline}}{Cost_{baseline}}
% \end{equation}
% while $Cost_{baseline}$ is 16 entry SRAM for VC, and for effective baseline router, $Cost_{system}$ is 32 entry SRAM for VC. Therefore its $CostRatio_{addition}$ is 100\%. However, for policy-based router, it only has it $CostRatio_{addition}$ as 25 \%. The hardware cost of a policy-based router is four-time less than the effective baseline router.

% Moreover, the actual router will have a more complicated and more profound packet buffer in one VC. Therefore the hardware cost gain of the policy-based router over effective baseline router can be way more than four times. If we need to accommodate the extreme case, then for the same assumed example, $CostRatio_{addition}$ for effective router is 300\%, with VCs as [32, 32, 32, 32]. Then the policy-based router will have hardware cost that is at least \textbf{12.15} times less than the effective baseline router. From the above illustrative example, we address the gain of the learned policy-based system, whose overhead is only a very small size SRAM. The gain for dynamic traffic situation can be easily addressed. Then, we emphasize on the gain for our VC allocation situation. The potential of it to be implemented in a more complicated and more extensive NoC system is high. 

%     The system we use is a Intel Xeon Platium 8164 CPU, 2.00 GHz with 26 cores. Our baseline system is a 64 nodes mesh Garnet 2.0. The runtime of our baseline system is 120 msec as mention previously. We compute there Energy Cost Ratio (ECR) as
% \begin{equation}
% ECR = P_{CPU}\frac{T_{learn}}{T_{baseline}}
% \end{equation}
% while $P_{CPU}$ is the power of our program, $T_{baseline}$ is the runtime of our baseline ststem, and $T_{learn}$ is the runtime of the system with learning method. Therefore, 
% \begin{equation}
% ECR_{baseline} = 1
% \end{equation}
% and $ECR_{learn}$ of different algorithms can be computed from \ref{table:2}. We can then compute their additional ECR (AECR) as an indication of energy overhead as 
% \begin{equation}
% AECR = ECR_{learn} - ECR_{baseline}
% \end{equation}
% The AECR of different algorithm is recorded in \ref{table:energy}.

% To compute the ratio of performance gain over energy overhead. We define this ratio as the Effective Peformnace Gain 
% \begin{equation}
% EPG = \frac{Perf_{learn}-Perf{baseline}}{ECR_{learn} - ECR_{baseline}}
% \end{equation}
% Therefore in S1, S2
% \begin{equation}
% EPG = \frac{throughput_{learn}-throughput_{baseline}}{ECR_{learn} - ECR_{baseline}}
% \end{equation}
% and in S3
% \begin{equation}
% EPG = \frac{-latency_{learn}-(-latency_{baseline})}{ECR_{learn} - ECR_{baseline}}
% \end{equation}


% However, We could deliver some thumps-up rule for the trade-off decision. For the scenario as our dynamic traffic, where the solution space is small, we could choose a more complex training. This could lead us faster to the optimal point. However, for the sceraio as our VC allocation, where we could only approach approximate solution, we could choose simpler algorithm. A simpler algorihtm with faster per runtime can shorten the time need for n

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% \subsubsection{Energy Cost}
% For the application 1: 

% For the application 2:

% For the application 3:


==> table/s3.tex <==

% \begin{table}[]
% \scalebox{0.7}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
%           & \multicolumn{3}{c|}{GA}    & \multicolumn{3}{c|}{PEPG}  & \multicolumn{3}{c|}{CMAES}  \\ \hline
%           & $Ep_{0}$ & $Ep_{50}$ & Impr. & $Ep_{0}$ & $Ep_{50}$ & Impr. & $Ep_{0}$ & $Ep_{50}$ & Impr.  \\ \hline
% Tornado    & 4.35  & 4.53       & +4.66 & 4.16  & 4.35       & +4.57 & 4.19  & 4.62       & +10.26 \\ \hline
% Shuffle    & 5.88  & 6.13       & +4.25 & 6.27  & 5.83       & +7.55 & 5.90  & 6.23       & +5.60  \\ \hline
% BitReverse & 4.94  & 5.02       & +1.74 & 4.93  & 5.17       & +4.87 & 4.94  & 5.13       & +3.88  \\ \hline
% BitRotate  & 6.44  & 6.55       & +1.72 & 6.13  & 6.6        & +7.67 & 6.35  & 6.51       & +2.55  \\ \hline
% Neighbor   & 14.81 & 15.12      & +2.10 & 15.03 & 15.33      & +2.03 & 14.20 & 15.08      & +6.20  \\ \hline
% Uniform    & 4.80  & 4.83       & +0.62 & 4.79  & 4.84       & +1.04 & 4.79  & 4.84       & +1.04  \\ \hline
% \end{tabular}}
%  \vspace{0.30cm}
% \caption{Throughput of the NoC with EA-based VC allocation in different traffic from gem5}
%  \vspace{-0.30cm}
% \label{table:s3}
% \end{table}

==> table/s4.tex <==
% \begin{table}[]
% \scalebox{0.7}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
%           & \multicolumn{3}{c|}{GA}     & \multicolumn{3}{c|}{PEPG}  & \multicolumn{3}{c|}{CMAES}  \\ \hline
%           & $Ep_{0}$  & $Ep_{50}$ & Impr. & $Ep_{0}$ & $Ep_{50}$ & Impr. & $Ep_{0}$  & $Ep_{50}$ & Impr. \\ \hline
% BC        & 25.56  & 25.61     & -0.19 & 25.76 & 25.72      & -0.16 & 25.56  & 25.57      & -0.08 \\ \hline
% BFSCC     & 25.60 & 25.58     & -0.09 & 25.64 & 25.62      & -0.07 & 25.63 & 25.58      & -0.18 \\ \hline
% Component & 25.39  & 25.36     & -0.13 & 25.43 & 25.37      & -0.24 & 25.44 & 25.45      & -0.35 \\ \hline
% BFS       & 25.54 & 25.51     & -0.12 & 25.80 & 25.66      & -0.54 & 25.61 & 25.46      & -0.50 \\ \hline
% kcore     & 25.96  & 25.68      & -1.09 & 25.66 & 25.61      & -0.19 & 25.64 & 25.566     & -0.28 \\ \hline
% PageRank  & 25.386 & 25.332     & -0.21 & 25.61 & 25.56      & -0.19 & 25.62  & 25.58      & -0.16 \\ \hline
% Radii     & 25.32 & 25.26     & -0.21 & 25.36 & 25.33      & -0.12 & 25.32 & 25.262     & -0.21 \\ \hline
% \end{tabular}}
% \vspace{0.30cm}
% \caption{Latency reduce of NoC with ES-based VC allocation in different traffic}
% \label{table:s4}
% \vspace{-0.30cm}
% \end{table}

==> table/time.tex <==

% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%                                                   & $\mathbf{Time_{S1}}$ & $\mathbf{Time_{S2_Tr}}$ & $\mathbf{Time_{S2_VC}}$ & $\mathbf{Time_{S3}}$ \\ \hline
% QL                                        & 178.1                                  & 137.6                                 & $N/A$                                  & $N/A$                       \\ \hline
% SARSA                                     & 162.0                                  & \textbf{133.6}                                  & $N/A$                                  & $N/A$                        \\ \hline
% E-SARSA                                            & 173.4                        & 139.9                         & $N/A$                                 & $N/A$                      \\ \hline
% \multicolumn{1}{|c|}{GA}   & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{l|}{147.2}             & 140.6                        \\ \hline
% \multicolumn{1}{|c|}{PEPG}   & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{l|}{147.4}             & 140.2                        \\ \hline
% \multicolumn{1}{|c|}{CMAES} & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{l|}{147.6}            & \textbf{133.8}                        \\ \hline
% \end{tabular}
% \vspace{0.30cm}
% \caption{The cost of training time (Seconds) for different policy learning techniques over interconnect environment for single iteration }
% \vspace{-0.30cm}
% \label{table:time}
% \end{table}
% \vspace{-0.3cm}
